DCN V2: Improved Deep & Cross Network and Practical Lessons for Web-scale Learning to Rank Systems

Learning effective feature crosses is the key behind building recommender systems. However, the sparse and large feature space requires exhaustive search to identify effective crosses. Deep & Cross Network (DCN) was proposed to automatically and efficiently learn bounded-degree predictive feature interactions. Unfortunately, in models that serve web-scale traffic with billions of training examples, DCN showed limited expressiveness in its cross network at learning more predictive feature interactions. Despite significant research progress made, many deep learning models in production still rely on traditional feed-forward neural networks to learn feature crosses inefficiently. In light of the pros/cons of DCN and existing feature interaction learning approaches, we propose an improved framework DCN-V2 to make DCN more practical in large-scale industrial settings. In a comprehensive experimental study with extensive hyper-parameter search and model tuning, we observed that DCN-V2 approaches outperform all the state-of-the-art algorithms on popular benchmark datasets. The improved DCN-V2 is more expressive yet remains cost efficient at feature interaction learning, especially when coupled with a mixture of low-rank architecture. DCN-V2 is simple, can be easily adopted as building blocks, and has delivered significant offline accuracy and online business metrics gains across many web-scale learning to rank systems at Google.

==> DCN - arxiv (long version) (4)/research_questions.tex <==
\section{Research Questions}
\label{sec:research_qs}
We are interested to seek answers for these following research questions:

\begin{itemize}[leftmargin=2.5em]
    \item[\bf RQ1]  When would feature interaction learning methods become more efficient than ReLU-based DNNs? What's the role of each component in the cross network?
    \item[\bf RQ2]  How does the feature-interaction component of each baseline perform without integrating with DNN? 
    \item[\bf RQ3]  How does the proposed mDCN approaches compare to the baselines? Could we achieve healthier trade-off between model accuracy and cost through mDCN and the mixture of low-rank DCN?
    \item[\bf RQ4]  Could cross network replace typical ReLU layers?
    \item[\bf RQ5] How does the settings in mDCN affect model quality?
    \item[\bf RQ6] Is mDCN capturing important feature crosses? Does the model provide good understandability?
\end{itemize}

==> research_questions.tex <==
\section{Research Questions}
\label{sec:research_qs}
We are interested to seek answers for these following research questions:

\begin{itemize}[leftmargin=2.5em]
    \item[\bf RQ1]  When would feature interaction learning methods become more efficient than ReLU-based DNNs? What's the role of each component in the cross network?
    \item[\bf RQ2]  How does the feature-interaction component of each baseline perform without integrating with DNN? 
    \item[\bf RQ3]  How does the proposed mDCN approaches compare to the baselines? Could we achieve healthier trade-off between model accuracy and cost through mDCN and the mixture of low-rank DCN?
    \item[\bf RQ4]  Could cross network replace typical ReLU layers?
    \item[\bf RQ5] How does the settings in mDCN affect model quality?
    \item[\bf RQ6] Is mDCN capturing important feature crosses? Does the model provide good understandability?
\end{itemize}
